On the Efficacy of Differentially Private Few-shot Image Classification

There has been significant recent progress in training differentially private (DP) models which achieve accuracy that approaches the best non-private models. These DP models are typically pretrained on large public datasets and then fine-tuned on private downstream datasets that are relatively large and similar in distribution to the pretraining data. However, in many applications including personalization and federated learning, it is crucial to perform well (i) in the few-shot setting, as obtaining large amounts of labeled data may be problematic; and (ii) on datasets from a wide variety of domains for use in various specialist settings. To understand under which conditions few-shot DP can be effective, we perform an exhaustive set of experiments that reveals how the accuracy and vulnerability to attack of few-shot DP image classification models are affected as the number of shots per class, privacy level, model architecture, downstream dataset, and subset of learnable parameters in the model vary. We show that to achieve DP accuracy on par with non-private models, the shots per class must be increased as the privacy level increases. We also show that learning parameter-efficient FiLM adapters under DP is competitive with learning just the final classifier layer or learning all of the network parameters. Finally, we evaluate DP federated learning systems and establish state-of-the-art performance on the challenging FLAIR benchmark.

==> bib_strings.tex <==
\newcommand{\aaai}[1]{Proceedings of the {#1} AAAI Conference on Artificial Intelligence (AAAI)}
\newcommand{\assets}{Proceedings of the International ACM SIGACCESS Conference on Computers and Accessibility (ASSETS)}
\newcommand{\bmvc}{Proceedings of the British Machine Vision Conference (BMVC)}
\newcommand{\cvpr}{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}
\newcommand{\eccv}{Proceedings of the European Conference on Computer Vision (ECCV)}
\newcommand{\iccv}{Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)}
\newcommand{\iclr}[1]{Proceedings of the {#1} International Conference on Learning Representations (ICLR)}
\newcommand{\icml}[1]{Proceedings of the {#1} International Conference on Machine Learning (ICML)}
\newcommand{\icra}{Proceedings of the IEEE International Conference on Robotics and Automation (ICRA)}
\newcommand{\ijcv}{International Journal of Computer Vision (IJCV)}
\newcommand{\iros}{Proceedings of the IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)}
\newcommand{\jmlr}{Journal of Machine Learning Research (JMLR)}
\newcommand{\neurips}[1]{Proceedings of the {#1} Annual Conference on Neural Information Processing Systems (NeurIPS)}
\newcommand{\pami}{IEEE Transactions on Pattern Analysis and Machine Intelligence (PAMI)}
